Spectral Function Space Learning and Numerical Linear Algebra Networks for Solving Linear Inverse Problems

We consider solving a probably ill-conditioned linear operator equation, where the operator is not modeled by physical laws but is specified via training pairs (consisting of images and data) of the input-output relation of the operator. We derive a stable method for computing the operator, which consists of first a Gram-Schmidt orthonormalization of images and a principal component analysis of the data. This two-step algorithm provides a spectral decomposition of the linear operator. Moreover, we show that both Gram-Schmidt and principal component analysis can be written as a deep neural network, which relates this procedure to de-and encoder networks. Therefore, we call the two-step algorithm a linear algebra network. Finally, we provide numerical simulations showing the strategy is feasible for reconstructing spectral functions and for solving operator equations without explicitly exploiting the physical model.

==> Makefile <==
MAIN = AspFriSch24_preprint1

.PHONY: default full final clean check whoareyou help

default:
	pdflatex --file-line-error $(MAIN).tex

full:
	latexmk -pdf --file-line-error $(MAIN).tex

clean:
	latexmk -c $(MAIN).tex
	rm -f $(MAIN).bbl $(MAIN).run.xml $(MAIN).thm $(MAIN).pdf

bib:
	$(eval AUX := $(shell mktemp -d))
	latexmk -gg -pdf -f -interaction=nonstopmode -jobname=extract -pdflatex="/usr/bin/pdflatex --file-line-error --shell-escape --synctex=1 %O '\def\extract{}\input{%S}'" -output-directory=${AUX} ${MAIN}.tex
	biber --output_format=bibtex --output_resolve -O ${AUX}/extract.bib ${AUX}/extract
	echo "\n%% Warning: This file is autogenerated, editing might be futile.\n" > csc.bib
	cat ${AUX}/extract.bib >> csc.bib
	rm -rf ${AUX}

check:
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN).tex

whoareyou:
	@echo $(MAIN)

help:
	@echo ""
	@echo "make targets are:"
	@echo ""
	@echo "  default (default):"
	@echo "    just builds the tex file (without bibliography)"
	@echo ""
	@echo "  full:"
	@echo "    builds the tex file (with bibliography)"
	@echo ""
	@echo "  final:"
	@echo "    extracts the bibliography into a local bib file"
	@echo "    creates an $(MAIN)_final.tex file using the extracted bib data"
	@echo ""
	@echo "  clean:"
	@echo "    cleans up temporary files"
	@echo ""
	@echo "  (check):"
	@echo "    used by the papercheck deamon, same as full but doesn't halt on error"
	@echo ""
	@echo "  (whoareyou):"
	@echo "    used by the papercheck daemon to identify this Makefile"
	@echo ""


